Harnessing Heterogeneity: Learning from Decomposed Feedback in Bayesian Modeling

There is significant interest in learning and optimizing a complex system composed of multiple sub-components, where these components may be agents or autonomous sensors. Among the rich literature on this topic, agent-based and domain-specific simulations can capture complex dynamics and subgroup interaction, but optimizing over such simulations can be computationally and algorithmically challenging. Bayesian approaches, such as Gaussian processes (GPs), can be used to learn a computationally tractable approximation to the underlying dynamics but typically neglect the detailed information about subgroups in the complicated system. We attempt to find the best of both worlds by proposing the idea of decomposed feedback, which captures group-based heterogeneity and dynamics. We introduce a novel decomposed GP regression to incorporate the subgroup decomposed feedback. Our modified regression has provably lower variance -- and thus a more accurate posterior -- compared to previous approaches; it also allows us to introduce a decomposed GP-UCB optimization algorithm that leverages subgroup feedback. The Bayesian nature of our method makes the optimization algorithm trackable with a theoretical guarantee on convergence and no-regret property. To demonstrate the wide applicability of this work, we execute our algorithm on two disparate social problems: infectious disease control in a heterogeneous population and allocation of distributed weather sensors. Experimental results show that our new method provides significant improvement compared to the state-of-the-art.

==> application.tex <==
\section{Other Applications}


==> backup.tex <==
\begin{theorem}[Theorem 1 provided by \citeauthor{srinivas2009gaussian} 2009]\label{thm:regret_bound}
Let $\delta \in (0,1)$ and $\beta_T = 2 \log(|\mathcal{X}| t^2 \pi^2 / 6 \delta )$.
Running GP-UCB with $\beta_t$ for a sample $f$ of a GP with mean function zero and bounded variance $k(\boldsymbol{x},\boldsymbol{x}) \leq 1$, we obtain a regret bound of $\mathcal{O}(\sqrt[]{T \gamma_T \log |\mathcal{X}|})$ with high probability. Precisely,
\begin{equation}\label{ineq:unnormalized_gpucb_regret_bound}
\text{Pr}\big\{ R_T \leq \sqrt[]{C_1 T \beta_T \gamma_T} ~\forall T \geq 1 \big\} \geq 1 - \delta
\end{equation}
where $C_1 = 8 / \log (1 + \sigma^{-2})$ and $\gamma_T = \max_{A \subset \mathcal{X}: |A| = T} I(y_A;f_A)$ is the maximum information gain of $T$ samples.
\end{theorem}
%They also proved, with certain kernels, the maximum information gain $\gamma_T$ is sublinear, resulting the regret bound to be sublinear too, which implies the no-regret property.

In our case, the individual kernels are bounded $k_j(\boldsymbol{x}, \boldsymbol{x}') \leq 1$.
But the entire kernel function $k(\boldsymbol{x}, \boldsymbol{x}') = \sum\limits_{j=1}^J g_j(\boldsymbol{x}) k_j(\boldsymbol{x}, \boldsymbol{x}') g_j(\boldsymbol{x}')$ has to be normalized by a constant factor $B^2$:
\begin{equation*}
k(\boldsymbol{x}, \boldsymbol{x}) \leq \sum\limits_{j=1}^J \max\limits_{\boldsymbol{x} \in \mathcal{X}} g^2_j(\boldsymbol{x}) = \sum\limits_{j=1}^J B_j^2 = B^2
\end{equation*}
where $B_j = \max\limits_{\boldsymbol{x} \in \mathcal{X}} |g_j(\boldsymbol{x})|$ and $B^2 = \sum B_j^2$.
Therefore, the regret bound in Theorem \ref{thm:regret_bound} can be normalized as:
\begin{equation}\label{ineq:normalized_gpucb_regret_bound}
\text{Pr}\big\{ R_T \leq \sqrt[]{C_1 T \beta_T B^2 \gamma_T} \quad \forall T \geq 1 \big\} \geq 1 - \delta
\end{equation}
where the information gain $I(y_T; f_T)$ can be written as:
\begin{equation*}
I(y_T; f_T) = \frac{1}{2} \sum\limits_{t=1}^T \log (\frac{\sum\limits_{j=1}^J g_j^2(\boldsymbol{x}_t) (1 + \sigma^{-2} \sigma_{i,t-1}^2 (\boldsymbol{x}_t)) }{\sum\limits_{j=1}^J g_j^2(\boldsymbol{x}_t)})
\end{equation*}
and $\gamma_T = \max\limits_{|x_T| = T, x_T \subset \mathcal{X}} I(y_T; f_T)$

==> flu.tex <==


\begin{figure}
    \includegraphics[width=0.45\textwidth]{figure/SEIS-model.pdf}
    \caption{MCF-SEIS Model with transition populations $A,B,C,D,E,F$ refer to the transition populations from states to states in the next year. {\color{red} probability TODO}}
    \label{fig:seis-model}
\end{figure}

\subsubsection{Flu Prevention {\color{red} TO BE MODIFIED!}}
The MCF-SIS (susceptible-infected-susceptible) model has two goals: to enable both realistic population dynamics and efficient optimization \cite{wilder132018preventing}.
The population is segmented into $n$ groups, referring to age group because disease transmission patterns for infection vary with age \cite{suen2015cost}.
We denote the number of susceptible people in each age group at time $t$ as the vector $S^t$ where $S^t_i$ indicates the susceptible population of group $i$.
Similarly, vectors $E^t$ and $I^t$ respectively refer to latent population and infected population at time $t$.
The total population at time $t$ can be written as $N^t = S^t + E^t + I^t$.

The transition of these states is illustrated in Figure \ref{fig:seis-model}.
The population change from susceptible is characterized by:
\begin{align*}
&A = S^t_i (1 - \mu^t_i) (1 - \gamma^t_i), &C = S^t_i (1 - \mu^t_i) \gamma^t_i
\end{align*}
where $\gamma^t_i = \sum\limits_{k=1}^n \beta_{ki} \frac{I^t_i}{N^t_i}$ is the infection probability of group $i$ with $\beta_{ki}$ being the disease transmission probability from group $k$ to group $i$.
Changes from latent and infected in Figure \ref{fig:seis-model} are also provided as following:
\begin{align*}
&B = I^t_i (1 - d^t_i) \boldsymbol{x}_{t,i}, &F = I^t_i (1 - d^t_i) (1 - \boldsymbol{x}_{t,i}) \\
&D = E^t_i (1 - \mu^t_i) (1 - \alpha^t_i), &E = E^t_i (1 - \mu^t_i) \alpha^t_i
\end{align*}
where $\boldsymbol{x}_{t,i}$ is the clearance rate at time $t$ and group $i$, which is also the probability that infected people in group $i$ get cured.
And $\alpha^t_i$ is the activation rate from latent state to infected state.
This model also considers the death rate of susceptible and latent people $\mu^t_i$ and of infected people $d^t_i$.
Migration from other cities can also be incorporated as the incoming population to different states: $\tilde{S}^{t}_{i}, \tilde{E}^{t}_{i}, \tilde{I}^{t}_{i}$.

In short, the population at time $t+1$ can be written as the summation of individual parts in Figure \ref{fig:seis-model}: $S^{t+1}_{i+1} = A + B + \hat{S}^t_i, E^{t+1}_{i+1} = C + D + \hat{E}^t_i, I^{t+1}_{i+1} = E + F + \hat{I}^t_i$.
All of these are analytical, so we can compute the future disease spread in all the following years with this model.

==> gp_figure_copy.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[height=2.8cm, width=5.8cm]{figure/entire_prior.png}
        \caption{Target function $f = f_1 + f_2$ and its sampled values}
        \label{fig:prior_samples}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[height=2.8cm, width=2.8cm]{figure/0_2_over_2.png}
        \includegraphics[height=2.8cm, width=2.8cm]{figure/1_2_over_2.png}
        \caption{Decomposed functions $f_1, f_2$ and their posteriors of GP regression.}
        \label{fig:decomposed_samples}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[height=2.8cm, width=5.8cm]{figure/comparison.png}
        \caption{The posteriors of decomposed GP regression and GP regression}
        \label{fig:entire_gpr}
    \end{subfigure}
    \caption{Illustration of decomposed GP regression (Algorithm \ref{alg:decomposed_gpr}) and comparison with GP regression (Algorithm \ref{alg:entire_gpr}).
    Decomposed GP regression shows a smaller average variance (0.878 v.s. 0.943) and a closer estimation to $f$. 
	\label{fig:decomposed_gpr}
	}
\end{figure*}

==> old_intro.tex <==

{\color{red} [old intro:}
Gaussian process has been widely applied to machine learning and non-parametric approximation.
In the multi-armed bandit setting, GP-UCB \cite{srinivas2009gaussian} was proposed to maximize the cumulative reward by optimally balancing between exploration and exploitation.
In general, in the policy determination problem {\color{red} to cite}, we consider each policy as an input and the reward (penalty) as the output, where we are aiming to maximize (minimize).
One concrete example is flu prevention {\color{red} to cite}.
The input is a yearly policy and the output is the total infected population in the following year.
We are aiming to find the optimal yearly policy which can minimize the total infected population.
Another example is apparent temperature (heat index).
The input is the sensor location and the output is the apparent temperature there.
Our goal here is to find the location with highest apparent temperature.
All the above examples involve the challenge to predict the outcome of unseen policy and location.
We usually call this type of problems as blackbox optimization: given an unknown function with certain smoothness assumption, the goal is to find the optimal solution by sampling in the input space.

In this paper, we focus on using Gaussian process regression (\cite{rasmussen2004gaussian}) to do approximation.
%Gaussian process regression is a very popular non-parametric method widely used to approximate the target function based on previous samples.
The approximation relies on the existing samples and the smoothness assumption (kernel function) to the target function.
Therefore it can draw conclusion to the unseen samples.
The value at an unseen sample is a Gaussian distribution with mean and variance, which depend on the values of existing samples and smoothness condition.
Previously, GP-UCB algorithm \cite{srinivas2009gaussian} is introduced to the bandit setting.
Similarly, it only requires the smoothness assumption to the target function but it can incorporate with noisy observation.
This advantage allows GP-UCB algorithm to be applied in many different fields ({\color{red} to cite!}) even if we do not have any prior knowledge.
Among GP-UCB idea, information is a very important part in function approximation and optimization.
The regret bound is directly related to the information gain and is proved to be sublinear while satisfying certain conditions.
Sublinear regret implies the average regret tends to 0, which also implies the convergence to the optimal solution.

However, in most of the real-world scenarios, we usually can further observe some side information while sampling.
For example, in the flu prevention case, although the objective value is the total infected population, we may be able to observe the age-wise infected population as well.
In the apparent temperature case, we are able to measure features like temperature, humidity, and wind speed.
If we know how these side information contributes to the objective value, we can take advantage on this prior knowledge.
In other word, if we know that the objective value is a composition of these features and we also have access to these features, then we can approximate these features by Gaussian process regression first.
After finishing the approximation, we can reconstruct the objective value by the approximation of features.
From the information perspective, we are using more information to reproduce the .
Intuitively, we should be able to achieve a more accurate approximation.

Flu prevention, as our main motivation, provides a more concrete illustration.
As mentioned above, we can observe the age-wise infected population while sampling and we know the total infected population is just the summation of all age-wise infected population.
So rather than approximating the total infected population, approximating each age-wise infected population turns to be more reasonable and informative.
We can then reconstruct the total infected population by simply summing up the approximation to the age-wise infected population.
This idea fully utilizes the side information revealed while sampling.

In this paper, we first prove that: with the help of the side information, we can get a better estimate by using Gaussian process regression.
This result indicates that if we can decompose the target function into several subfunctions where we can observe their realization in the previous samples, then approximating each subfunction individually first and assembling the result to get the target function will be better than directly approximating the entire function.
Secondly, we apply this idea to multi-arm bandit problem.
A stochastic bandit problem is an online learning problem where at each step a learning agent chooses one of ground items, and then observes stochastic reward of this item as a payoff.
A combinatorial semi-bandit problem allows multiple accesses to the ground items subject to combinatorial constraint, and then observes stochastic rewards of these items and receive their sum as a payoff.
We consider a similar concept to semi-bandit problem: {\bf non-combinatorial semi-bandit problem}.
Here, in the non-combinatorial semi-bandit setting, we assume each time we can only choose one item.
But instead of only observing the reward of this item, we can observe some side information (hidden variables) of this item.
We propose an algorithm adopting side information in the non-combinatorial semi-bandit setting.
Further we prove the no-regret property of our algorithm, implying the convergence to the optimal solution.
Lastly we compare our algorithm using side information and the previous GP-UCB algorithm without using side information.
The result shows that our algorithm requires less samples to reduce the average regret to certain level, or equivalently to achieve certain solution quality.
This concludes the advantage of adopting side information.
{\color{red} ]}
%A popular model to disease problem is SIS (susceptible-infected-susceptible) population model \cite{wilder132018preventing}.
%SIS model is a population model which encodes the transmission between age groups and provides an analytical estimate to the infected population in each groups.
%With the help of the analytical model, we can do optimization on this analytical model.
%However, the limitation to this method is the testimony of the disease model.
%Even though there are some hyper-parameters that can be adjusted, the model is still quite restricted and can be far from the real-world disease.
%For example, randomness can never be encoded in the analytical deterministic model.
%Therefore, in order to cover this short end, we can approximate the difference between SIS model and the real flu by Gaussian process regression.
%Moreover, the side information encoded in both SIS model and real flu can help us approximate the difference faster, leading to a smaller sample complexity and thus to converge to the optimal solution faster.

%Another popular idea is to consider the entire function as a blackbox function.
%Our problem becomes a blackbox optimization problem.
%In the previous literature, there are different ways to deal with the optimization over an unknown function.
%Gaussian process regression \cite{rasmussen2004gaussian} is a commonly used non-parametric Bayesian method.
%According to the previous samples, Gaussian process regression can update the belief to the target function.
%The only assumption to this method is smoothness (Gaussian process kernel).
%Thus Gaussian process regression is also a very general technique in both approximation and optimization.
%However, its generality is a double-edged sword.
%The convergent rate of Gaussian process regression is extremely slow, which makes it become a very expensive method compared to surrogate based algorithm.

%The idea of side information, or equivalently the decomposition of the target function, can be applied to many different scenarios.
%If the learner has certain prior knowledge to the objective function, which can be thought as a hybrid of the analytical model and non-parametric Gaussian process model.
%Instead of directly using the analytical model, we assume the model is imperfect and try to apply Gaussian process regression to learn the error terms of this analytical model.
%In other words, we are standing on the shoulder of analytical model and then apply GP method to further improve the accuracy of the approximation.
%For example, in every sample to the Tuberculosis prevention, we can observe both total infected population (our objective function) and also individual infected population at each age.




%In our Tuberculosis prevention setting, both simulation and field test are usually time-consuming and very expensive.
%Moreover, the observation may also be noisy, which means the function itself is an unknown stochastic function instead of a deterministic function.
%Normally, we can consider the target function to be a blackbox stochastic function, and our goal is to approximate this blackbox function by existing samples and thus optimize it.
%However, the traditional gradient descent method does not apply since we do not have a gradient oracle to the function.
%Although we can estimate the gradient by local sampling, it becomes too expensive since estimating the gradient in a high dimensional space requires even more samples, resulting in a huge burden to the runtime.
%Based on these limitations, how to efficiently approximate and optimize the unknown function becomes a common interest in many different fields.







